Can Deep Neural Networks Predict Data Correlations from Column Names?

Recent publications suggest using natural language analysis on database schema elements to guide tuning and profiling efforts. The underlying hypothesis is that state-of-the-art language processing methods, so-called language models, are able to extract information on data properties from schema text. This paper examines that hypothesis in the context of data correlation analysis: is it possible to find column pairs with correlated data by analyzing their names via language models? First, the paper introduces a novel benchmark for data correlation analysis, created by analyzing thousands of Kaggle data sets (and available for download). Second, it uses that data to study the ability of language models to predict correlation, based on column names. The analysis covers different language models, various correlation metrics, and a multitude of accuracy metrics. It pinpoints factors that contribute to successful predictions, such as the length of column names as well as the ratio of words. Finally, \rev{the study analyzes the impact of column types on prediction performance.} The results show that schema text can be a useful source of information and inform future research efforts, targeted at NLP-enhanced database tuning and data profiling.

==> sections/implications.tex <==
\section{Implications and Outlook}
\label{sec:implications}

Predicting correlations without expensive data analysis is useful in various scenarios. In the following, we connect our results to application scenarios around database tuning. Section~\ref{sub:usecase} discusses a corresponding use case. Also, in Section~\ref{sub:extensions}, we discuss extensions of the prediction methods used in the experiments presented so far.

\subsection{Use Case in Database Tuning}
\label{sub:usecase}

We predict correlations based on column names. The resulting correlations are less interesting from the perspective of data exploration. If correlations can be predicted from column names alone, they relate to commonsense knowledge and do not yield new and interesting insights about specific data sets. However, in the introduction, we have partially motivated our experiments with use cases around database tuning. In this section, we make those motivations more concrete by sketching out a use case for correlation prediction in the context of query optimization. Note that specifying or evaluating a corresponding solution in detail is beyond the scope of this publication. Merely, we want to elaborate on our initial references to potential use cases.

\tikzstyle{component}=[fill=blue!10, rectangle, draw=black, font=\itshape]
\tikzstyle{dataflow}=[->, ultra thick]
\tikzstyle{io}=[font=\bfseries]

\begin{figure}
    \centering
    \begin{tikzpicture}
        \node[io] (data) at (-2,0) {Data};
        \node[io] (schema) at (2,0) {Schema};
        \node[component] (danalysis) at (-2,-1) {Data Analysis};
        \node[component] (sanalysis) at (2,-1) {NLP Analysis};
        \node[component] (model) at (0,-2) {Cost and Cardinality Model};
        \node[component] (optimizer) at (0,-3) {Query Optimizer};
        \node[io] (query) at (-3,-3) {Query};
        \node[io] (plan) at (3,-3) {Plan};
        \draw[dataflow] (data) -- (danalysis);
        \draw[dataflow] (schema) -- (sanalysis);
        \draw[dataflow] (danalysis) -- (model);
        \draw[dataflow] (sanalysis) -- (model);
        \draw[dataflow] (model) -- (optimizer);
        \draw[dataflow] (query) -- (optimizer);
        \draw[dataflow] (optimizer) -- (plan);
    \end{tikzpicture}
    \caption{Sketch of NLP-enhanced query optimizer.}
    \label{fig:nlptuning}
\end{figure}

Figure~\ref{fig:nlptuning} sketches out a system that uses NLP-based correlation prediction for query optimization. A query optimizer generally tries to map a query to a near-optimal query plan. To do so, it must estimate processing costs for plan candidates. Processing cost depends however on the cardinality of intermediate results. Data correlations can throw off estimation which, at least according to standard models~\cite{Selinger1979}, assumes uniform data and independent query predicates~\cite{Gubichev2015}. 

NLP-based correlation prediction could become one additional source of information in cost estimation. For instance, it could be used to target efforts in collecting data statistics. Instead of collecting statistics on all possible column pairs, collection could focus on column pairs that are likely correlated, based on their column names. According to our results, a corresponding approach would not find all but most of the correlated column pairs (while significantly reducing analysis overheads). Our results indicate that integrating initial correlation results, obtained while analyzing a specific data set, could improve further predictions on that data further (Hypothesis~\ref{hyp:quality}). Here, NLP-backed correlation prediction may help to lower overheads in collecting statistics used by more traditional cost models. This can make query optimization more reliable.

Recent work explores the use of machine learning for cost and cardinality estimation in the context of query optimization~\cite{Kipf2018, Park2020, Sun2020}. In that context, NLP-based correlation prediction could serve as an additional input feature. Especially for new data sets, for which few queries have been processed so far, it could serve for initialization until more training data has been observed. We plan to explore corresponding approaches in our future work.

%Having a mechanism that detects correlations with high confidence, without requiring expensive data analysis, could help making query optimizers more reliable. As shown in Figure~\ref{fig:nlptuning}, NLP-based analysis of schema elements could become one additional source of information, used for cost estimation. The results obtained in this paper demonstrate that NLP-based correlation prediction can be done with reasonable accuracy in many scenarios, in particular if column names are long enough (which is easy to test). Hence, the possibility to consider corresponding features for cost and cardinality estimation seems interesting. This applies even more as machine learning has recently been demonstrated to work well for cost and cardinality estimation for query optimization. In this context, NLP-based analysis results become one more feature whose weights can be learned via training. 

The systems outlined above only serve as an illustration, showing at a high level of abstraction how correlation prediction can become useful for database tuning. The applicability of NLP-based correlation predication is however not restricted to those use cases. Next, we discuss several extensions to the prediction methods used so far.

\subsection{Extensions}
\label{sub:extensions}

The prediction methods evaluated in the previous sections use only column names as features. While already informative, we see several possibilities to expand the scope of input features further. A first possibility is to use the name of the data set or any text associated with the data. Many data sets, e.g.\ on Kaggle, come with so called ``data dictionaries''. Those dictionaries explain semantics of columns in more detail, typically using one or multiple paragraphs of text. Clearly, this text often yields information beyond what can be inferred from column names alone. However, trying to exploit such text via NLP leads to new challenges. It is still difficult to accurately interpret longer text documents, even though significant progress has been made recently~\cite{Zaheer2020, Yang2020a, Beltagy2020}. We plan to evaluate some of those recently proposed methods on data-related text documents, as opposed to short column names, in our future work.

Up until now, we have treated correlation prediction as a binary classification problem (i.e., we classify column pairs into correlated and non-correlated pairs). This requires setting thresholds defining which degree of correlation qualifies. Alternatively, we can model correlation prediction as a regression problem. E.g., instead of predicting whether the $R$ value of specific columns exceeds a threshold, we can try to predict $R$ directly. We plan to explore this option in future work.

The aforementioned extensions change the problem model. Beyond that, there are several optimizations of the current approach that we have not yet exploited. For instance, our approach uses raw column names as input, only replacing underscores by spaces. There are other methods that are often used to construct column names from words. For instance, we observed several cases of ``camel caps'' notation. Resolving such cases in a pre-processing step could yield further performance improvements.

==> sections/replies.tex <==
\twocolumn

\section*{Summary of Changes}

Dear reviewers and dear meta-reviewer,
\vspace{0.25cm}

Thank you for the detailed comments and suggestions! The revision addresses all points made by the reviewers. Please find more details below. Changes in the paper are marked in \rev{red}. Beyond the revised paper, more experiments are available in an \textbf{extended technical report}. This report is available here:

\begin{center}
    \url{http://itrummer.org/drafts/CorrelationPrediction.pdf}
\end{center}

\subsection*{Meta-Review}

\rew{Further improve the presentation to help readers better understand the work referring to (R1.D1-D11, R2.D5-D6)}

\begin{answer}
    The presentation was updated, as requested by the reviewers.
\end{answer}

\rew{Provide more technical details according to \\ (R2.W1, R2.D1, R2.D4,R3.D1,R3.D3)}

\begin{answer}
    The revised papers contains clarifications with regards to the points raised by the reviewers.
\end{answer}


\rew{Further enhance experiments by considering \\ (R3.W2, R3.D2,R3.D4,R3.D6)}

\begin{answer}
    The revised paper contains additional experiments. More experiments are available in the extended technical report.
\end{answer}


\subsection*{Reviewer \#1}

\rew{D1) This work seems to use a lot of space to justify the idea that columns are semantically relevant to the data they contain... I do not find this idea needing much statement at all. I think it is only academics who name all their columns "c1" "c2" "c3" etc. Probably sufficient to say "good practice and common sense means that most column names are meaningful, but of course there are rare exceptions which we are not concerned with here"}

\begin{answer}
    Thanks for the suggestion! The revision contains the wording at the start of the introduction, shortening the text in the process (e.g., by replacing a corresponding footnote).
\end{answer}


\rew{D2) I chuckled a little when the introduction mentioned "several recent publications" with citations to more work done by the paper's authors. This is not a problem, but there's no reason to make this look like something it isn't! "My previous work in this area uncovered a natural question: can large language models..." (this happens twice in the 2nd column of the paper :D )}

\begin{answer}
    Ok! The revision clarifies authorship in the introduction and in the related work section.
\end{answer}


\rew{D3) "as justified by prior work, pairwise column correlations..." I think looking at more than two columns would turn the problem from quadratic to exponential, right? It isn't about what is useful in practice, it just isn't feasible to do. Or am I missing something?}

\begin{answer}
    Indeed, detecting more than pairwise correlations is expensive. The revised Section~3.1 clarifies that fact. At the same time, it cites prior work claiming that considering correlation between column pairs resolves most of the selectivity estimation error in an experiment. The revised Section~3.1 now quotes the relevant sentence from the prior paper as well.
\end{answer}


\rew{D4) "only up to 100 columns" how do you pick the 100 columns? To avoid the problem of many-column databases dominating the metrics, couldn't you just normalize each metric by the number of columns in each dataset?}

\begin{answer}\label{ans:uptotencolumns}
    The revised paper clarifies in Section~3.1 that the column pairs are formed by considering (up to) the first ten columns of each table. If going beyond 100 column pairs per data set, the number of data sets that can be analyzed with a given time budget decreases. As the number of column pairs grows quadratically in the number of columns, few of the wide tables on Kaggle (sometimes featuring several tens up to even a hundred columns) may account for a number of column pairs that is comparable to the total number of column pairs in the current benchmark. Limiting the number of column pairs per data set is a way to increase the number of data sets, and therefore diversity of topics covered, that can be analyzed within a reasonable amount of time.
\end{answer}


\rew{D5) my understanding of 3.1 is that we have a bunch of continuous measures of correlation, and we're going to pick a threshold for each measure that we decide is "correlated" and anything under that threshold is "uncorrelated." The methodology for picking the cutoff value is a p-value of 5\%. But I am not sure the p-value interpretation really holds here -- for Pearsons, for example, the p-value is computed assumes heteroskadasticity, normally-distributed measurement errors, etc. all of which seem a little suspect here. At minimum, the distributional assumptions behind these p-values should be stated.}

\rew{But I think the whole interpretation of the p-value is wrong on a deeper level. One read of the p-value is that it is the probability that two data columns would be as correlated as they are if they were drawn randomly. But in reality, two data columns might have a *ground truth* non-zero correlation that is under the threshold (e.g., only a subset of the data is highly-correlated, or two parts of the data are inversely-correlated with each other).}

\rew{Why not just use the actual measures of correlation as the targets of your modeling, turning the problem into a regression problem?}

\begin{answer}
    Turning it into a regression problem is an interesting extension. The regression problem seems more difficult than the classification variant (having a perfect predictor for the regression problem, e.g., predicting Pearson correlation values, yields a perfect predictor for the classification problem as well, but not vice-versa). At the same time, having predictors for the classification variant is already useful (e.g., for prioritizing data profiling). The revised paper discusses the different variants at the end of Section~3.1.
\end{answer}


\rew{D6) I think a reasonable concern with Kaggle data + \\ Albert/Roberta/Distilbert is twofold:}

\rew{A) that we don't know if the pre-training data for those language models included information about the Kaggle datasets. A lot of the Kaggle datasets get discussed elsewhere online, or are re-hashes of old datasets (so the date of the Kaggle dataset is meaningless in this sense). Are you 100\% sure these LMs never saw any info about these Kaggle datasets? If so/not, I think it should be discussed.}

\rew{B) Kaggle datasets are not independent. Sometimes, the same task gets posted multiple times or with slight variations (like the presence or absence of additional features). This would be a big problem for fine-tuning (test set leakage), but could also be skewing the results from the pre-trained models with no fine-tuning as well. How do we know that this isn't a problem?}

\begin{answer}
    Agreed, those points should be discussed in the paper. The revised paper discusses those issues at the beginning of Section~3.1 and addresses questions that relate to similarities between training and test data in Section~6. In short: having references to Kaggle data sets in the (pre-)training data is insufficient, it would take information on data correlation between their columns to be useful (considering the correlation metrics used in this paper). As this information is relatively specific, it seems unlikely that pre-training data covers a large number of test cases. The results in Section~6 are representative for a predictor, trained on a subset of data sets and then applied to others. This corresponds to a realistic scenario in which one would benefit, indeed, from similarities between training and test data (this similarity can come in multiple forms, e.g., starting with common column names that are associated with similar semantics). In that sense, the reported results evaluate prediction quality in a realistic scenario.
\end{answer}


\rew{D7) In S5.3, what happened to hypothesis 3? Also, it would be nice if the hypotheses were presented closer to where they are actually evaluated, or at least if there was a clear marker for where to go to. Same for S6 and S7. Maybe just use a paragraph header when you go on to a particular hypothesis?}

\begin{answer}
    The revised Section~5.3 now explicitly refers to Hypothesis~3. Also, the revised paper puts all hypotheses directly before the text discussing them. Thanks for the suggestion!
\end{answer}


\rew{D8) In S7 for hypothesis 7, how do we know that shorter column names are not simply more likely to be placeholders or noise? "f4" or "feature 4" is definitely something I've seen on kaggle. Seems like longer strings might just have a lower probability of being placeholders.}

\begin{answer}
    Hypothesis~7 is consistent with a scenario in which shorter column names tend to be placeholders. In general, the hypothesis does not make any claims about the nature of shorter column names. Placeholders could be defined in multiple ways. If we define them as text strings, followed by numbers, they would be associated with a low ratio of English words. However, the ratio of English words in column names seem to matter less, according to the results discussed in the second half of Section~7. The revised paper discusses the possibility of placeholder column names directly before introducing Hypothesis~8.
\end{answer}


\rew{D9) Looking at H7 and H8 together, I wonder if you could create a classifier that takes in an embedding of a column name and predicts whether or not accuracy will be high or not. Sort of like a model to guess how well the other model is working. You could then analyze the classifier to try and see what the "secret" is, or use the classifier as a way to calibrate confidence for the predictor.}

\begin{answer}
    That is true. The revised Section~7 discusses this possibility at the end of the section.
\end{answer}


\rew{D10) S9 seems really incomplete. It seems like the start of an idea for a much broader, much bigger system that is much more advanced than what you previously proposed. But I am not sure it really belongs here. I think the space would be better used to make the plots bigger, add x-axis labels, etc.}

\begin{answer}
    Thanks for the suggestion! Former Section~9 was now moved to the extended technical report, thereby creating more space for plots and added text.
\end{answer}


\rew{D11) Expanding on the first point, these graphs are kinda rough. I understand that the legend is being used instead of an x-axis to make things less crowded, but they all seem too small and difficult to read. The grid lines are nearly fully covered by many bars. I think if you drop or shorten S9 you can give the plots a lot more space to breath. A lot of the plots could also be combined into a single figure, like F18 and F19.}

\begin{answer}
    The revised paper contains significantly larger plots (the height was increased). Also, the plots contain the actual numbers inside of the bars, making it easier to read plots precisely. Indeed, moving Section~9 to the extended technical report created the required space. Also, the revised paper merges multiple plots into the same figure (as sub-figures), e.g., in Section~6, 7, and 8.
\end{answer}


\subsection*{Reviewer \#2}

\rew{W1. I'm not sure whether the author has ensured that there's no "leak" of labels from the training set to the test set. For example, a table may have a correlated pair of column names that shows in the training set, but another table may have the same correlated pair of column names that shows in the test set. And the model just "remembers" this pair instead of learning the semantics behind them.}

\begin{answer}
    Strictly speaking, one test case is characterized by the names of a column pair, as well as by the associated data, which determines the label (i.e., correlated or uncorrelated, according to the current correlation metric). Section~6 shows results for scenarios in which column pairs appearing in training and test data are taken from different data sets. Of course, different data sets on Kaggle may have similarities in terms of column names as well as associated data. However, the reported results represent a practical scenario in which predictors are trained on a subset of data sets, then applied to others. Section~6 discusses similarities between training and test data towards the end.
\end{answer}

%Even if the same column names appear in two different tables, the associated data is in general different. This means that the corresponding labels, i.e., whether correlated or not, can be different, too. 


\rew{W2. This is more of (i.e.,  a suggestion than a weak point - Can the author include the data type from the language model as well? It seems that data type can be simple to include since it's directly available from the meta-data. And the data type may also provide useful information to determine the column correlation.}

\begin{answer}
    Thanks for the suggestion! The revision contains a new section, Section~9, that trains language models to use column types, in addition to column names (see Figure~\ref{fig:typed}). For most scenarios, adding types improves prediction performance slightly.
\end{answer}


\rew{D1. How are the 100 column pairs of each table selected? 100 can be a very small subset of all possible column pairs if the table has a large number of columns. How does the author ensure that the selected pairs are representative and contain correlated columns if there are any in the table?}

\begin{answer}
    Up to the first ten columns of a table are selected to form column pairs. The goal of restricting the number of column pairs per table is to analyze more data sets within a reasonable analysis time (also see Answer~\ref{ans:uptotencolumns}). Guaranteeing to select correlated column pairs if they appear in a table would require analyzing all possible column pairs, thereby defeating the purpose of the restriction. Selecting correlated column pairs if they appear in a table may also lead to a benchmark in which correlated column pairs are over-represented, compared to the actual data. The revised Section~3.1 clarifies how column pairs are selected. 
\end{answer}


\rew{D2. How does the author fine-tune a language model to predict the correlation between columns? I.e., how a language model that predicts the probability of the next word converts to a classification model that predicts whether two columns are correlated?}

\begin{answer}
    Decoder models like GPT typically predict the probability of the next token. This evaluation uses encoder models like Roberta. In their raw form, those models associate input tokens with high-dimensional vectors. Additionally, a task-specific layer is added that maps vectors to the desired output. For classification problems, this last layer typically maps one of the output vectors (typically the vector associated with the first token) to scores for different classes. The class with the highest score is the assumed classification result. Indeed, the original version of the paper lacked details on the type of models used. The revised version explains encoder models and how they are used for classification in Section~5.1. Thanks for the suggestion!
\end{answer}


\rew{D3. It seems that 20\% of training data does not reduce the model performance significantly compared to 80\%. I'm wondering how small the amount of training data can be without significantly impacting the model performance? Also out of curiosity, is it possible to directly use the pre-trained language models without fine-tuning? If so, what the performance would be?}

\begin{answer}
    The revised paper reports results for a zero-shot scenario, i.e., using no training data for correlation prediction whatsoever (see Figure~\ref{fig:pearsonScenarios}, \ref{fig:spearmanScenarios}, and \ref{fig:theilsUscenarios}). The results show clearly the need for fine-tuning on the specific prediction task.
\end{answer}


\rew{D4. Is there any correlation trend related to column types? For example, is any particular column type that is easier to have correlation/predict correlation?}

\begin{answer}
    The revised paper contains a new section, Section~\ref{sec:types}, showing breakdowns of prediction performance metrics by the types of the correlated columns. Indeed, prediction performance varies across different column types.
\end{answer}


\rew{D5. How do existing data profiling tools determine which columns to prioritize during profiling? Are there any existing methods other than random?}

\begin{answer}
    The revised related work section (Section~2.2) contains more details on how existing profiling tools (specifically for correlation detection) prioritize profiling overheads (based on data samples).
\end{answer}


\subsection*{Reviewer \#3/\#4}

\rew{W1. It is not clear how many more column names can be discovered within a fixed time interval when the NLP tools direct a correlation analyzer compared to the state of the art (see D1).}

\rew{D1. A key motivator for this paper is that an NLP-driven approach reduces the computation time required to find column correlations. While Section 9 shows that NLP tools effectively find correlated column names, it is unclear how long the inference period is. How does this method compare to subsampling a small number of rows from the relevant columns and analyzing the correlation for the sample? It would be good to show these results given the accuracy-computation trade-offs made by Albert and Distilbert.}

\begin{answer}
    Following the suggestion by Reviewer~1, the relevant section was moved to the appendix of the extended technical report (Appendix~A). The revised section in that report now reports inference time (which is low, compared to data analysis overheads, even for the small tables used for analysis). At the same time, the section discusses the use of sub-samples and contrasts the given approach. Note that those two methods (analyzing column names and analyzing sub-samples) are not mutually exclusive and could be used together in a more sophisticated profiling tool. This is however beyond the scope of this paper.
\end{answer}


\rew{W2. The comparison baseline is simple. A more robust baseline is required to establish the superiority of an NLP-directed approach (see D2).}

\rew{D2. The paper establishes that an NLP-driven approach is superior to a randomized approach for finding column correlations. However, the baseline used earlier in the paper considered Jaccard similarity, which seems like a more realistic baseline.}

\begin{answer}
    (As suggested by Reviewer~1, the section on NLP-enhanced profiling was moved to Appendix~A in the extended technical report.) The extended technical report contains results for a baseline that is based on Jaccard similarity, rather than language models (see Figure~\ref{fig:tuning}).
\end{answer}


%\rew{W3. The experiment sections would benefit from small refinements for increased clarity and breadth.}



\rew{D3. If the NLP predictor is highly confident that two columns are correlated, is the correlation value higher than if it is less confident?}

\begin{answer}
    The extended technical report contains a new appendix section (Appendix~B) that analyzes dependencies between prediction confidence and correlation strength.
\end{answer}


\rew{D4. In Section 9.3, is a separate benchmark run conducted for only the "large tables"? Or, do these results mean that of the detected correlations across all tables, they tend to be found in the large tables?}

\begin{answer}
    This is a separate benchmark, using only a subset of the tables that have a large number of columns. The revised technical report clarifies that.
\end{answer}


\rew{D5. Section 6 shows that training using some column names and correlations from a dataset improves the performance in predicting correlations among other columns in the dataset. Does this mean significant overlap (e.g., Jaccard similarity) exists among column name tokens for correlated columns?}

\begin{answer}
    The extended technical report contains results, linking Jaccard similarity to the strength of correlation (see Appendix~B, in particular Figure~\ref{fig:predictionVsCorrelation}). While Jaccard similarity is zero for many column pairs, making it less effective as a heuristic to guide profiling, columns with high Jaccard similarity are more likely to be correlated indeed.
\end{answer}


\rew{D6. Small fixes: The paper uses lowercase BERT names (e.g., Distilbert) throughout, but the conclusion uses "DistilBERT". Section 5.1 states that Distilbert shows significant speedups with very moderate loss in quality. This phrasing is somewhat ambiguous.}

\begin{answer}
    The revised paper corrects the capitalization in the conclusion. Also, it rephrases the statement in Section~5.1.
\end{answer}

